Linear-Time Verification of Data-Aware Dynamic Systems with Arithmetic

Combined modeling and verification of dynamic systems and the data they operate on has gained momentum in AI and in several application domains. We investigate the expressive yet concise framework of data-aware dynamic systems (DDS), extending it with linear arithmetic, and provide the following contributions. First, we introduce a new, semantic property of "finite summary", which guarantees the existence of a faithful finite-state abstraction. We rely on this to show that checking whether a witness exists for a linear-time, finite-trace property is decidable for DDSs with finite summary. Second, we demonstrate that several decidability conditions studied in formal methods and database theory can be seen as concrete, checkable instances of this property. This also gives rise to new decidability results. Third, we show how the abstract, uniform property of finite summary leads to modularity results: a system enjoys finite summary if it can be partitioned appropriately into smaller systems that possess the property. Our results allow us to analyze systems that were out of reach in earlier approaches. Finally, we demonstrate the feasibility of our approach in a prototype implementation.

==> A5-1_example_cg.tex <==
\subsection{Examples for constraint graphs}

\begin{example}[Monotonicity constraints]
We consider the MC-\mydds $\BB_1$ from \figref{examples}, where we add state names and
action labels to simplify notation below:
\begin{center}
\begin{tikzpicture}[node distance=24mm]
\node[state] (1) {$b_1$};
\node[state, right of=1, double] (2) {$b_2$};
\draw[edge] ($(1) + (-.4,0)$) -- (1);
\draw[edge, rounded corners] (1) -- node[above,action]{$a_1\:[x^w > y^r]$} (2);
\draw[edge, rounded corners] (2) -- ($(2) - (0,.5)$)
  -- node[below,action]{$a_2\:[y^w > x^r]$}  ($(1) - (0,.5)$)  -- (1);
\end{tikzpicture}
\end{center}
We have $V = \{x,y\}$, and consider $\BB_1$ as a \mydds over $\mathbb Q$.
For simplicity, let $\CC = \emptyset$. 
The constraint graph $\CG$ can be constructed according to 
\defref{constraint graph} as follows:\\
$\bullet$ The initial node is $(b_1, \phi_0)$, where we assume that
$\phi_0 = C_{\alpha_0} = (x=0 \wedge y=0)$.
\\
$\bullet$ 
The successor of $(b_1, \phi_0)$ after executing action $a_1$ is 
$(b_2, \phi_1)$ for some $\phi_1$ such that
$\phi_1 \equiv \update(\phi_0, a_1)$. 
According to the proof of \thmref{mc}, we can compute $\phi_1$ by
applying quantifier elimination to $\update(\phi_0, a_1)$, to
obtain a quantifier-free MC formula over variables $V$:
\begin{align*}
\update(\phi_0, a_1) &= 
 \exists \vec V_0 C_{\alpha_0}(\vec V_0) \wedge  \trans{a_1}(\vec V_0, \vec V) \\
 & = \exists x_0 y_0. x_0=0 \wedge y_0\,{=}\,0\wedge x\,{>}\,y_0 \wedge y\,{=}\,y_0\\
 &\equiv x > 0 \wedge y\,{=}\,0
\end{align*}
Note that the names of the quantified variables are irrelevant, as they are immediately removed.
We here use numbered vectors $\vec V_0, \vec V_1, \vec V_2, \dots$ merely to
emphasize progress.\\
%
$\bullet$ 
Similarly, the successor of $(b_2, \phi_1)$ by executing action $a_2$ is
$(b_1, \phi_2)$ for some $\phi_2$ such that
$\phi_2 \equiv \update(\phi_1, a_2)$.
\begin{align*}
\update(\phi_1, a_2) &= 
 \exists \vec V_1 \phi_1(\vec V_1) \wedge  \trans{a_2}(\vec V_1, \vec V) \\
 & = \exists x_1 y_1. x_1\,{>}\,0 \wedge y_1\,{=}\,0 \wedge x\,{=}\,x_1 \wedge y\,{>}\,x_1\\
 &\equiv x\,{>}\,0 \wedge y\,{>}\,x
\end{align*}
Note that the result of quantifier elimination need not be unique.
For instance, $\phi_2 $ could be equivalently chosen as 
$x\,{>}\,0 \wedge y\,{>}\,x \wedge y\,{>}\,0$.
However, when restricting to variables $V$ and constants that occur in 
$\alpha_0$, guards of $\BB$, and $\CC$ (as implied by the proof of \thmref{mc}),
there are only finitely many choices. Hence the constraint graph computation would
even converge with a nondeterministic quantifier elimination procedure, if the \mydds has finite summary.
In practice a deterministic procedure can be assumed.\\
%
$\bullet$ 
The successor of $(b_1, \phi_2)$ by executing action $a_1$ is
$(b_2, \phi_3)$ for some $\phi_2$ such that
$\phi_3 \equiv \update(\phi_2, a_1)$.
\begin{align*}
\update(\phi_2, a_1) &= 
 \exists \vec V_2 \phi_2(\vec V_2) \wedge  \trans{a_1}(\vec V_2, \vec V) \\
 & = \exists x_2 y_2.\:x_2\,{>}\,0 \wedge y_2\,{>}\,x_2 \wedge x\,{>}\,y_2 \wedge y\,{=}\,y_2\\
 &\equiv x\,{>}\,y \wedge y\,{>}\,0
\end{align*}
%
$\bullet$ 
The successor of $(b_2, \phi_3)$ by executing action $a_2$ is
$(b_1, \phi_4)$ for some $\phi_4$ such that
$\phi_4 \equiv \update(\phi_3, a_2)$.
\begin{align*}
\update(\phi_3, a_2) &= 
 \exists \vec V_3 \phi_3(\vec V_3) \wedge  \trans{a_2}(\vec V_3, \vec V) \\
 & = \exists x_3 y_3.\:x_3\,{>}\,y_3 \wedge y_3\,{>}\,0 \wedge x\,{=}\,x_3 \wedge y\,{>}\,x_3\\
 &\equiv x > 0 \wedge y > x
\end{align*}
Hence $\phi_4=\phi_2$, so that the computation reached a fixed point, and we obtain the following constraint graph:
\begin{center}
\begin{tikzpicture}[node distance=24mm]
\tikzstyle{node}=[rectangle, rounded corners, inner sep=3pt, draw, scale=.8, thick]
\node[node] (1) {$b_1,\phi_0$};
\node[node, right of=1] (2) {$b_2, \phi_1$};
\node[node, right of=2] (3) {$b_1, \phi_2$};
\node[node, right of=3] (4) {$b_2, \phi_3$};
\draw[thick,->] ($(1) + (-.8,0)$) -- (1);
\draw[thick,->] (1) -- node[above,action]{$a_1$} (2);
\draw[thick,->] (2) -- node[above,action]{$a_2$} (3);
\draw[thick,->] (3) to[bend left] node[above,action]{$a_1$} (4);
\draw[thick,->] (4) to[bend left] node[below,action]{$a_2$} (3);
\end{tikzpicture}
\end{center}
\end{example}



==> macros-style.tex <==
\makeatletter
\g@addto@macro\normalsize{%
\setlength{\abovecaptionskip}{3pt}
\setlength{\belowcaptionskip}{-10pt}
\setlength\abovedisplayskip{3pt}
\setlength\belowdisplayskip{3pt}
\setlength\abovedisplayshortskip{3pt}
\setlength\belowdisplayshortskip{3pt}
%\setlength\topsep{2pt}
}
\makeatother


